The Mathematical Foundations for Mapping Policies to Network Devices (Technical Report)

A common requirement in policy specification languages is the ability to map policies to the underlying network devices. Doing so, in a provably correct way, is important in a security policy context, so administrators can be confident of the level of protection provided by the policies for their networks. Existing policy languages allow policy composition but lack formal semantics to allocate policy to network devices. Our research tackles this from first principles: we ask how network policies can be described at a high-level, independent of firewall-vendor and network minutiae. We identify the algebraic requirements of the policy mapping process and propose semantic foundations to formally verify if a policy is implemented by the correct set of policy-arbiters. We show the value of our proposed algebras in maintaining concise network-device configurations by applying them to real-world networks.

==> Firewall path algebra - tech report/abstractions.tex <==
\section{\uppercase{Abstract policies}}
\label{sec:abstractions}
\vspace{-2mm}
% 1. HL policy must be decoupled from network using abstractions.
Abstractions are key to constructing high-level policies.
A good policy abstraction should capture the underlying 
concepts naturally and concisely. For instance, a policy may be arbitrated using one or more network devices.
A good abstraction should decouple {\em what} is arbitrated from {\em how} it is arbitrated.

% TODO: comment on potential complexity of policy graph (ie, full mesh)?
% high-level policies in general can be expressed using an endpoint-pair and an edge (relationship)
A simple abstraction that is commonly used to decouple policy from the network is {\em (endpoint-group, edge)} \cite{ranathunga2015V,bartal1999,soule2014,prakash2015}.
An {\em endpoint} is a grouping of elements based on common physical or logical properties- \eg a subnet, a user-group, a collection of servers, {\em etc.}
An {\em endpoint} is also the smallest unit of abstraction a policy can be applied to.
An {\em edge} specifies the relationship between the endpoints, \ie it describes what communication is allowed between the endpoints.
An edge typically consists of a Boolean predicate (\ie classifier) that matches traffic packet header details to perform some action.
An edge from endpoint $S1$ to $S2$ with predicate $R$ means that a correct implementation should act in some specified way toward traffic from all members (\eg hosts) in $S1$ to those in $S2$ satisfying $R$.

Consider the example network in Figure \autoref{fig:network}, our high-level policy might be -- ``we want to measure all HTTPS flows from $S1$ to $S4$".
This intent can be expressed using the (endpoint-group, edge) abstraction as \verb|p:=S1| $\rightarrow$ \verb|S4 : collect https|, where $p \in \mathcal{P}$ is an element of the possible space $\mathcal{P}$ of policies.

% 2. Mapping HL policy to devices is complicated by the device topology.
We now want to map the policy to enforcing devices (\ie arbiters). It looks naively easy. Just implement the policy on arbiter $F$. However, the problem is in general more complicated.
For example, consider policy from $S1$ to $S2$. If arbiter $A$ captures flows described by policy $p_A$ and likewise $p_B$, then the combination is
$p_{A \cap B}$ because the policy expresses that flows be collected but load balancing across the two paths could result in either being used by a given packet.

For another example, consider policy from $S2$ to $S3$. If arbiters $C$ and $D$ capture flows described by policy $p_C$ and $p_D$ respectively, then
the combination would yield their {\em union} because both arbiters in the path are used for flow collection. 
So, when mapping policies to network devices, they must be composed in a way that preserve the topology-specific semantics.

We will, in general, denote the policy composition resulting from parallel routes as $p_A \oplus p_B$ and that resulting from serial routes as $p_A \otimes p_B$.
In this example, $p_A \oplus p_B=p_{A \cap B}$ and $p_C \otimes p_D=p_{C \cup D}$.
Note though, the meaning of $\oplus$, $\otimes$ are policy-context dependent.

% talk about redundancy what if F fails (policy S1->S4)? - we would want some redundancy and still be able to collect flows
The problem of mapping our high-level policy $p$ (from $S1$ to $S4$) to network devices, may even be more complicated than simply implementing the policy on $F$.
What happens if $F$ drops out? Surely we would still want to collect HTTPS flows that traverse the redundant paths from $S1$ and $S4$ (\eg path via $S2$ and $S3$). So, $p$ must also be mapped to the policy arbiters along the path $S1-S2-S3-S4$, to cater for this redundancy. 
But then, should we map the policy to all of these arbiters or a subset of them?

Given the parallel routes between $S1$ and $S2$ it is easy to see that we need to map $p$ to both $A$ and $B$ to preserve the semantics of $\oplus$.
But, when arbiters are in series (\eg $C,D$) we have the choice of mapping policy to both or just one to preserve the semantics of $\otimes$.
Mapping to both may be unnecessary and inefficient and arbiters may have limits on their capabilities.

\begin{figure}[t!]
\captionsetup{aboveskip=8pt}
\centering
\subfigure[Network topology.] % caption for subfigure a
{
	\includegraphics[scale=0.32]{network1.pdf}
	\label{fig:network}	
}
\hspace{0.1cm}
\subfigure[Policy graph of (a).] % caption for subfigure b
{
	\includegraphics[scale=0.32]{abs_model.pdf}
	\label{fig:abs_model}
}
\caption{Example network consisting of four endpoints ($S1-S4$) and six policy arbiters ${A,B,...,F}$ (a). The corresponding policy graph is shown in (b) with these endpoints and 
policy edges ($E1,E2,...,E6$) between them.}
\label{fig:network_abs}
\end{figure}

\begin{figure}[t!]
\captionsetup{aboveskip=8pt}
\centering
\subfigure[Network of 3 endpoints connected to a single device.] % caption for subfigure a
{
	\includegraphics[scale=0.175]{hyper_edge_net.pdf}
	\label{fig:star}	
}
\hspace{0.3cm}
\subfigure[Policy hyper-graph model of (a).] % caption for subfigure b
{
	\includegraphics[scale=0.215]{hyper_edge_c.pdf}
	\label{fig:hyper}
}
\hspace{0.15cm}
\subfigure[Policy simple-graph model of (a).] % caption for subfigure b
{
	\includegraphics[scale=0.215]{simple_edge_c.pdf}
	\label{fig:simple}
}
\caption{Policy-graph definition alternatives.}
\label{fig:alternat}
\end{figure}

% how do we map policy in the star topology? 
The policy arbiters may not always be in series or parallel. For instance, consider the star-topology involving the endpoints $S3,S4$ and $S5$ in Figure \autoref{fig:star}. The question of how to map policy to topology gets interesting in this case. We could loosely map policy to arbiter $G$ using a {\em hyper-edge} $E7$ (Figure \autoref{fig:hyper}).
But, doing so adds to the complexity of the policy-graph and decreases it's precision.
For instance, it allows a $1:n$ relationship between hyper-edges and policies, so, we must track the policy of {\em every endpoint-pair} in a hyper-edge
to correctly map it's policy to network devices. Also, a hyper-edge could potentially map to a large portion of the network (\eg when interconnected to many endpoints), so, it's policy can be complex, difficult to understand and debug.

We can overcome these problems by using a simple-edge mapping instead (Figure \autoref{fig:simple}).
By doing so, we also gain significant benefits.
For one, the policy graph is simplified and it's precision is increased-- the $1:1$ relationship between edges and policies now mean we only need to track a single policy for each edge, to map policy accurately to devices. For another, our simplified abstraction {\em (endpoint-pair, edge)} 
behaves as a network-slice \cite{gutz2012}-- a piece of the network that can be programmed independently from the rest of the network -- so, debugging policy errors is easy. Moreover, users from distinct policy subdomains (\eg Engineering, Corporate Administration) can manage the network-slices (\ie policy-edges) applicable to their domain. 

% TODO: this is an important issue: use diagrams to illustrate (possibly under own heading) ?
We may also need to consider paths that consist of one more intermediate endpoints,
when implementing policy between an endpoint pair.
For instance, consider implementing a security policy $f:=$\verb|S1| $\rightarrow$ \verb|S3: http| in the network in Figure \autoref{fig:network}.
Once implemented on the arbiters (\ie firewalls), the policy should allow HTTP traffic flow from \verb|S1| to \verb|S3|.
But, the policy can only be deployed correctly if endpoints \verb|S2,S4| can route or forward HTTP traffic.

% 3. Mapping HL policy to devices is ALSO complicated by the endpoint traffic transitivity.
This ability of an endpoint to route or forward traffic can be restrictive.
For instance, in a security policy context, an endpoint can group systems (\eg hosts) with similar security requirements \cite{isa2007}.
So, high-risk systems can be grouped in to one endpoint and only {\em safe} traffic that originate and/or terminate at the endpoint is permitted by the security policy. 
Enabling this endpoint to transit-traffic could potentially expose the high-risk systems within to cyber attacks.
So, an endpoint's {\em traffic transitivity} capability must be considered in constructing valid device-paths between endpoints and
captured explicitly in the mapping process.
%So, an endpoint's {\em traffic transitivity} capability is also an important consideration in the policy mapping process.
%We will discuss this traffic transitivity in detail later in \autoref{sec:algebra}.
%To do so, \verb|S2,S4| must consist of routers or switches.

The intent of our high-level policy $p$ is to collect HTTPS flow data from $S1$ to $S4$.
Similarly, traffic measurement policies can be defined between any pair of endpoints in the network, so the corresponding
(endpoint-pair,edge) tuples collectively construct a {\em policy-graph} (Figure \autoref{fig:abs_model}).
Each (logical) edge in this graph maps to a physical network path comprising of policy arbiters and zero or more intermediate endpoints.
For instance, policy-edge $E4$ in Figure \autoref{fig:abs_model} implements our policy $p$.

%Mapping policy to network-devices is also constrained by the {\em traffic transitivity} (\ie routing) capabilities of the endpoints.
%For instance, a traffic measurement policy: \verb|S1| $\rightarrow$ \verb|S3: http|, can only be implemented if the endpoints \verb|S2| and \verb|S4| route HTTP traffic through to \verb|S3|. 
%So, an endpoint's ability to route traffic (\ie traffic transitivity) is also an important property to consider when mapping policy to network devices.
%We will discuss this traffic transitivity in detail later in \autoref{sec:algebra}.
% TODO:The notion of traffic transitivity depends on what a zone/endpoint really is=> are arbiters routers?

% elaborate the concept using a typical set of policies
%Restricting a $1:1$ mapping between edges and policies also highlights the role of {\em device interfaces}.
%We need to know, for instance, whether to implement a policy on input or output interfaces.
%So far, we have described some of the challenges faced when mapping policies to network-devices.
So far, we have described several key requirements of a policy-to-device mapping process.
We next illustrate these using more detailed examples involving a typical set of policies found in practice.
The examples also show the use of our {\em (endpoint-pair, edge)} abstraction in high-level policy description.
%Restricting a 1 : 1 mapping between edges and policies simplifies our base abstraction to {\em (endpoint-pair, edge)}.
%We illustrate its use for high-level policy specification by considering a typical set of policies found in practice.
%In the following, we present more detailed examples.
\vspace{-3mm}
% 4. Show how HL policy can be mapped to devices in different policy contexts
\subsection{Quality of Service (QoS) Policies}
\vspace{-3mm}
QoS policies can be used, for instance, to provide bandwidth guarantees for certain types of traffic.
The policy arbiters in this context, would commonly be QoS capable routers or switches.
Imagine we need to provision a minimum bandwidth of 100MB/s for HTTP traffic flow from $S1$ to $S4$ in Figure \autoref{fig:network}.
The high-level policy intent can be expressed using the endpoint-pair $S1$, $S4$ and an edge ($E4$) between them: \verb|min(S1| $\rightarrow$ \verb|S4 : http, 100MB/s)|.
In reality, similar QoS policies between any endpoint-pair can be expressed using the same policy-graph in Figure \autoref{fig:abs_model}.

% implications on policy when serial, parallel device topologies are used
Parallel and serial (QoS-device) topologies also have an impact on the end QoS policy.
Consider the parallel topology between $S1$ and $S2$ in Figure \autoref{fig:network}, if we assume $p_A$ and $p_B$ provide bandwidth guarantees
of $B1$ and $B2$ respectively, then with load balancing, the resultant QoS policy ($p_R$) 
can provide a total bandwidth guarantee $p_R=p_A \oplus p_B = sum(B1,B2)$.

When the devices are in series (\eg topology between $S2$ and $S3$ in Figure \autoref{fig:network}), the resultant policy provides a bandwidth guarantee given by $p_C \otimes p_D=min(B3,B4)$ where $B3,B4$ are the bandwidth guarantees provided by $p_C$ and $p_D$.

This example highlights how policies can be composed using the generic semantics $\oplus$ and $\otimes$ in different policy contexts.
The actual meaning of these operators is policy-type dependant.
For instance, in the traffic measurement policy example, $\otimes$ represented {\em union} while here
it has meaning of {\em minimum}.

% TODO: hyper-edge vs simple-edge for QoS policy representation
%	      : traffic transitivity implications
% 	      : problem with generic abstractions
We can see that endpoint traffic-transitivity also impacts the ability to implement a QoS policy correctly in the network.
For instance, consider policy \verb|min(S1| $\rightarrow$ \verb|S3 : http, 50MB/s)|, the required bandwidth
guarantee can only be provided if $S2,S4$ routes or forwards traffic to $S3$.
%( in addition to the network-paths explicitly described by arbiters. )
%TODO: what do we learn from these examples?
\vspace{-3mm}
\subsection{Security Policies}
\label{sec:sec}
\vspace{-3mm}
The security policies we consider here are access-control policies in a network.
The policy arbiters in this context, would be traffic filtering devices (\eg firewalls, SDN switches).
The endpoints could be zones or user groups.
Imagine we want to enable only SSH traffic from $S1$ to $S4$ (Figure \autoref{fig:network}). The high-level policy can be expressed using the endpoint-pair $S1$, $S4$ and an edge between them as \verb|S1| $\rightarrow$ \verb|S4: ssh| with an
implicit \verb|deny-all| in place.

% implications on policy when serial, parallel device topologies are used
When the traffic filtering devices are in parallel (\eg topology between $S1$ and $S2$ in Figure \autoref{fig:network}), the resultant security policy ($p_R$), has meaning- {\em all packets that can {\em possibly} be allowed through} -- and is the {\em union} of the packet sets allowed through by the individual devices. We take union conservatively because intrusions and attacks are usually carried out through permitted traffic.
So, if $p_A$ and $p_B$ allows packet sets $Q$ and $T$ respectively, then $p_R=p_A \oplus p_B = p_{Q \cup T}$.

When the devices are in series (\eg topology between $S2$ and $S3$), the resultant policy permits the {\em intersection} of the packet sets $V,W$ allowed by the policies of $C$, $D$ respectively -\ie  $p_R=p_C \otimes p_D = p_{V \cap W}$. 

With security policies, it is often useful to have endpoints that group systems with similar security requirements.
Doing so, allows to define a {\em single policy} for all members of an endpoint-- a clean and concise abstraction of network security.
But, a generic (endpoint-pair, edge) abstraction cannot capture such network-security specific policy concepts precisely.

So, we need concrete definitions for what an endpoint and an edge means for each policy context
to capture policy-specific intricacies.
We will show later how to define these concretely for security policies.
\vspace{-3mm}
\subsection{Traffic Measurement Policies}
\label{sec:measure}
\vspace{-3mm}
Traffic measurement policies can be used to implement, for instance, NetFlow (v9) on the example network shown in Figure \autoref{fig:network}.
The policy arbiters ${A,B,...,F}$ here, would be NetFlow capable devices (usually routers or switches).
The endpoints could be subnets or zones in the network.

% implications on policy when serial, parallel device topologies are used
When we considered the parallel routes between $S1$ and $S2$,
the resultant policy ($p_R$) with meaning--
{\em the flows that are guaranteed to be captured by the topology (without sampling)},
constitutes of the {\em intersection} of the packet sets of $A$ and $B$.
So, if $p_A$ and $p_B$ capture packet sets $Q$ and $T$ respectively, then $p_R=p_A \oplus p_B = p_{Q \cap T}$.

We also showed that when the devices are in series (\eg topology between $S2$ and $S3$ in Figure \autoref{fig:network}), the resultant policy captures the {\em union} of the packet sets $V, W$ captured by the policy of the devices $C$ and $D$ respectively, \ie  $p_R=p_C \otimes p_D = p_{V \cup W}$. 
% TODO: hyper-edge vs simple-edge for traffic measurement policy representation
%	      : traffic transitivity implications
% 	      : problem with generic abstractions

% 5. Policy mapping has parallels with routing
\smallskip
\smallskip
\noindent \textbf{\em Policy Mapping Vs Routing:} We can see that in mapping policies to network devices, our discussion above relates to network paths or routes.
This is no accident. The problem we aim to solve has many parallels with routing. But here,
\begin{itemize}
\item{we often look for all paths, not just best paths.}
\vspace{-1mm}
\item{we do not need to employ decentralised protocols. A logically-centralised implementation can offer a robust and efficient solution
as demonstrated in SDN \cite{anderson2014,foster2010,soule2014,prakash2015}.}
\end{itemize}

The aim in routing is to determine the path that optimises a given path-metric (\eg shortest-path routing finds
a path between endpoints with a minimum distance). Our target problem is different: we need to determine the set of arbiters in a network a given policy should be implemented on. So, constructing all feasible paths is crucial because, for instance, a security policy between two endpoints can only be correctly implemented (\eg to block all Telnet traffic) if all redundant paths between them are taken into account.

We also expect a relatively low number of endpoints (\eg in \autoref{sec:example} we will see this number is typically $< 25$ in a SCADA network),
through network grouping. As we will show in \autoref{sec:imp}, a low endpoint-count makes our policy-mapping algorithm computationally tractable.
So, a logically-centralised implementation can be considered. But, in routing, the number of endpoints (\eg individual gateways) can be high for a large network, so, distributed means to computing a solution is essential (requiring de-centralised protocols like OSPF, BGP) . Our policy-mapping algorithm can also be implemented distributedly if necessary.

%6. But routing algebra wouldn't work
Algebras have also been proposed in meta-routing \cite{griffin2013}, to provably choose paths that optimise various path-metrics.
But, these algebras {\em do not support specification of node properties}
such as traffic transitivity. Specification of link properties is possible and we could translate node properties to
link properties, but, the workaround is not elegant.
A better approach is to have an algebra that capture node properties explicitly.

%\smallskip
\smallskip
% 7. (endpoint-pair, edge) abstraction must be concretised to capture policy specific features 
% (ie derive a really useful HL policy description for each case), then it can be used
% for policy mapping
\noindent We described in \autoref{sec:sec}, the need to define endpoints and edges concretely for each policy context.
By doing so, we can incorporate the intricacies associated with each policy type.
We illustrate the idea next using security policies and their concretised (endpoint-pair, edge) abstraction- {\em the Zone-Conduit model}.
%which we also describe in detail 

\smallskip
\noindent \textbf{\em The Zone-Conduit Model}:
Lack of internal-network segmentation is a key contributor to the fast propagation of threats and attacks in a network \cite{byres2005}.
So, ANSI/ISA have proposed the {\em Zone-Conduit model} as a way of segmenting and isolating the various sub-systems in a SCADA network \cite{isa2007}.

A \textit{zone} is a logical or physical grouping of an organisation's
systems with similar security requirements so that a {\em single policy}
can be defined for all zone members. A \textit{conduit}
provides the secure communication path between two zones, enforcing
the policy between them \cite{isa2007}.
A conduit could consist of
multiple links and firewalls but, logically, is a single connector.

% the z-c model is a refined version of the (EP,edge) abstraction that captures security properties well.
It is easy to see that the Zone-Conduit model is a concrete instance of the (endpoint-pair, edge) abstraction for high-level security policy specification.
The zones and conduits are concrete definitions of endpoints and edges.
In defining them, important network-security characteristics such as {\em a single zone-policy}, are captured concisely.

The Zone-Conduit model abstracts {\em how} security policy is enforced, so users can focus on
{\em what} policy to enforce.
The model intuitively decouples policy from topology, so, high-level security policies 
can be described free of network and vendor intricacies. 

The ISA Zone-Conduit model in its original description lacks precision for policy specification. 
We use the extensions proposed in
\cite{ranathunga2015} to increase its precision, \eg we add Firewall-Zones to specify firewall-management policies.
%\autoref{fig:zcmodel} shows an example of this refined Zone-Conduit model adapted from a real SCADA network.
\iffalse
\begin{figure}[t!]
%\center
\captionsetup{aboveskip=8pt}
\centerline{\includegraphics[scale=0.3]{zone-cd2.pdf}}
\caption{Zone-Conduit model of a real SCADA network adapted from a case study \cite{ranathunga2015}. The model is a concrete instance of the (endpoint-pair, edge) abstraction where the zones are the nodes and the conduits are the edges.}
\label{fig:zcmodel}
\end{figure}
\fi

\begin{figure*}[t!]
\captionsetup{aboveskip=8pt}
\centering
\subfigure[Zone-Firewall model.] % caption for subfigure a
{
	\includegraphics[scale=0.36]{transitivity_zfw.pdf}
	\label{fig:vc1}
}
\hspace{0.8cm}
\subfigure[Firewall-path model of (a).] % caption for subfigure b
{
	\includegraphics[scale=0.37]{transitivity_zcd.pdf}
	\label{fig:vcf1}
}
\caption{Example of traffic packets traversing a single firewall interface twice. As shown by the path in red, if traffic from zone 1 to 2 is allowed to transit zone 3, 
firewall interface e0 is traversed twice. In this situation, the direct path from zone 1 to 2 is more efficient. So, we deem firewall path $A_{13}A_{32}$ invalid (\ie =$\phi$), since
$h(A_{13})=h(A_{32})=A$, where $h: F \rightarrow W$.}
\label{fig:fwloop}
\end{figure*}

\smallskip
\noindent \textbf{\em Zone-Conduit Policies}:
A conduit policy is essentially an ordered set of rules $[p_1,p_2,...,p_n]$ that act on packet sequences to accept, deny, or in some cases, modify them.
In our related work \cite{ranathunga2015V,ranathunga2015P}, we have identified properties and constraint required in a Zone-Conduit based policy description to make these rules vendor and device (\ie implementation) independent
and have rule-order independent semantics. 

To summarise, we adopt a security whitelisting model, \ie we restrict policies to express positive abilities\footnote{Refers to the ability to initiate or accept a traffic service.} and {\em deny all} inter-zone flows that are not explicitly allowed \cite{ranathunga2015V}. 
Doing so, renders the rule order irrelevant in a policy, 
allowing the policy to be converted consistently to different vendor firewalls. So, the underlying vendor can change without requiring policy alterations. Policy makers can also add or remove policy rules oblivious to the ordering of the rules. 
By being explicit, we also prevent services being accidentally enabled implicitly. 

\iffalse
\begin{figure}[t!]
\captionsetup{aboveskip=8pt}
\centering
\subfigure[Policy on a single conduit.] % caption for subfigure a
{
	\includegraphics[scale=0.3]{policy_c.pdf}
	\label{fig:pc1}	
}
\hspace{0.1cm}
\subfigure[Firewall paths of conduit in (a).] % caption for subfigure b
{
	\includegraphics[scale=0.3]{fw_c.pdf}
	\label{fig:fwc1}
}
\vspace{0.2cm}
%\hspace{0.1cm}
\subfigure[Directed-conduit policies equivalent to (a).] % caption for subfigure b
{
	\includegraphics[scale=0.3]{policy_dc.pdf}
	\label{fig:pdc1}
}
\hspace{0.1cm}
\subfigure[Directed-firewall paths of conduits in (c).] % caption for subfigure b
{
	\includegraphics[scale=0.3]{df_dc.pdf}
	\label{fig:dfdc1}
}
\caption{Example of how a conduit policy $p_0$ can be expressed using two directed-conduit policies $p_A$ and $p_B$. Conduits map to firewalls and directed-conduits map to directed-firewalls. }
\label{fig:dc1}
\end{figure}
\fi

\smallskip
\noindent \textbf{\em Directed- vs Undirected-Conduit Policy}:
The policy on an undirected-conduit can be expressed using two {\em directed-conduit} policies.
Directed-conduits are important in understanding how policy should
be implemented on device interfaces. For instance, consider implementing
a security policy $p:=Z1 \rightarrow Z2: https$ on the network shown in Figure \autoref{fig:vc1}.
An undirected-conduit can only map the policy to firewall interfaces $e1,e2$.
But, to implement the policy correctly, we additionally need to know if it should be implemented 
{\em inbound} or {\em outbound} on these interfaces. A directed-conduit provides this directionality.

However, analysis using directed-conduits can also lead to problems. For instance,
it seems feasible to implement our policy $p$ along the path highlighted in red in Figure \autoref{fig:vcf1}.
But further inspection of Figure \autoref{fig:vc1}, reveals that traffic packets traversing this path 
would require to traverse firewall interface $e0$ twice.

% TODO: explain why this is not just a looped path?

We invalidate such directed-conduit paths via a mapping
$h: F \rightarrow W$ where $F=\{directed \ firewalls\}$ and $W=\{firewalls\}$.
A directed-firewall in the Zone-Conduit graph $G=(Z,C)$ is defined as
\vspace{-2mm}
\begin{defn}[Directed firewall]
  A {\em directed firewall} $t_{ij}$ is a firewall $t \in W$ that filters traffic on directed-conduit $(i,j) \in C$.
  \label{def:directed_firewall1}
\end{defn}
\vspace{-2mm}
\noindent Then we can check if the directed-firewalls in a path map to the same physical firewall
(\ie $h(A_{13})=h(A_{31})=A$) and deem that path invalid.

\iffalse
%TODO: maybe incorporate elsewhere
A conduit policy may be implemented by a single or collection of firewalls.
So, we can define a mapping $q: C \rightarrow \mathcal{P}(W)$ where
$C=\{undirected \ conduits\}$, $\mathcal{P}$ is Power-set and $W=\{firewalls\}.$

We can extend the idea to directed-conduits and define mapping $v: D \rightarrow \mathcal{P}(F)$ where $D=\{directed \ conduits\}$,
$\mathcal{P}$ is Power-set and $F=\{directed \ firewalls\}.$

% also relate back the generic (EP,edge) abstraction to show how the above concepts are applicable in other policy contexts
It is easy to see that the definitions of the mappings $q$ , $v$ and $h$ above can be tailored to suit each policy context.
%For instance, with traffic measurement policies $q: C \rightarrow W$ and $v: D \rightarrow F$
%where $C=\{policy \ edges\}$, $W=\{policy \ arbiters\}$, $D=\{directed \ edges\}$ and $F=\{directed \ devices\}$. 
\fi

%paths that seem legit in the directed model may actually be invalid. 
%this can only be verified by referring to the undirected conduit model and its firewall mappings
% also direct conduits help identify how policy should be implemented 
%on the device interfaces (eg, inbound or outbound on a firewall interface)

%For instance, conduit-policy $p_0$ in Figure \autoref{fig:pc1} can be expressed using the directed-conduit policies $p_A$ and $p_B$ in Figure \autoref{fig:pdc1}.
% conduits map to firewalls, direct-conduits map to directed firewalls
%For instance, our example conduit-policy $p_0$ can be implemented by a single firewall $A$ (Figure \autoref{fig:fwc1}).


\iffalse
%TODO: remove?
But, when mapping policy to firewalls for implementation purposes, it may be necessary to
resolve down to a firewall-interface level. 
For instance, with traditional firewalls such as Cisco ASAs, the traffic filtering policies (\ie \ac{ACLs})
must be assigned to the firewall interfaces in appropriate directions to enforce policy correctly. 
So, we need a mapping with more resolution than what $T$ (above) provides.

For a policy-graph $G=(V,C)$, a directed-device can be defined as 
\begin{defn}[Directed device]
  A {\em directed device} $t_{ij}$ is a policy arbiter $t \in W$ on edge $(i,j) \in C$.
  \label{def:directed_device1}
\end{defn}
\vspace{-6mm}
\fi

\vspace{-7mm}

==> Firewall path algebra - tech report/algebra.tex <==
\section{\uppercase{Mapping Algebra}}
\label{sec:algebra}
\vspace{-3mm}
We now outline our proposed algebras to map high-level policy to network devices.
We start by making the distinction between {\em primary} and {\em secondary}
policy-edges, and then later show how the latter can be derived algebraically using the former.
\vspace{-2mm}
\subsection{Firewall-path Construction}
\label{sec:encoding}
\vspace{-3mm}
As we described earlier, a policy-edge enforces policy between two endpoints in a network.
A policy-edge can be classified as a {\em primary-} or a {\em secondary-edge} depending what
arbiters are implemented within.
A primary-edge can enforce policy {\em only} using policy arbiters.
A secondary-edge enforces policy using both arbiters and one or more additional endpoints.

We demonstrate the idea using security policies and the simple Zone-Conduit graph $G=(Z,C)$ in Figure \autoref{fig:vc50}. 
The firewall composition of each primary-conduit in the model is shown (Figure \autoref{fig:vcf51}).
The example secondary-conduit $C_{13}$ filters traffic flow from zone \verb|1| to \verb|3|, using several directed-firewalls
and transit zones \verb|2|, \verb|4|.
The set of all directed-conduits are given by $DC=\{C_{ij} \ | \ (i,j) \in C \}$.

%TODO: add how the label subscripts (eg, 12) maps to a firewall interface (eg, e0) 
% eg define a mapping from directed-firewalls (F) to fw interfaces (I): (1,2) -> (e0, e2) where Z1 is connected to e0 and Z2 connected to e2
% with FWZs only 1 interfaces is physical (other is MDI).
A policy-graph is essentially an automation that moves traffic packets from 
one endpoint to another using policy-edges. So, regular expressions (the natural language of finite automata),
can capture the packet-processing behaviour of this model; a path encoding is a concatenation of directed-devices (\ie policy-arbitration steps $pq$) 
and a set of paths is encoded as a union of paths.
Past work \cite{anderson2014} has shown, all single-path encodings stem from the Kleene star operator (*) on the set of directed-devices.
%all possible single-path encodings

In a security policy context, the automation means that a single firewall-path encoding is a concatenation of directed-firewalls.
Each path depicts a sequence of traffic filtering steps and is an element of $F^*$.

\begin{figure*}[t!]
\captionsetup{aboveskip=8pt}
\centering
\subfigure[Zone-Conduit model with primary and secondary conduits.] % caption for subfigure a
{
	\includegraphics[scale=0.4]{vc-zcd.pdf}
	\label{fig:vc50}
}
\hspace{0.8cm}
\subfigure[Firewall-paths of the primary-conduits in (a).] % caption for subfigure b
{
	\includegraphics[scale=0.4]{vc-zcdf1.pdf}
	\label{fig:vcf51}
	% original scale=0.257
}
\caption{Zone-Conduit model depicting primary-conduits $C_{ij}$ and a secondary-conduit $C_{13}$ enabled by the transit zones 2 and 4 shown in (a). The firewall-paths of the primary-conduits are shown in (b).}
\label{fig:zc50}
\end{figure*}

But, the Zone-Conduit model is a logical representation, so, every firewall-path encoding in $F^*$ may not be valid.
We follow the design principles below to filter-out invalid paths:
\vspace{-1mm}
\begin{itemize}
\item{non-elementary paths in the Zone-Conduit model must be {\em excluded}.}
% Looped paths simply waste resources and cause unnecessary delays.}
% TODO: should this be a lemma?
\vspace{-2mm}
\item{when traversing elementary Zone-Conduit paths, traffic packets shouldn't traverse a particular device interface more than once. 
So, for directed-firewalls $t_{ij},t_{jk} \in F$ the concatenation $t_{ij}t_{jk}$ is valid {\em iff} $h(t_{ij}) \neq h(t_{jk})$. 
We demonstrated the idea using the simple example in \autoref{fig:fwloop} earlier. }
\vspace{-2mm}
\item{traffic cannot flow through a non-transit zone. 
Typical zones this restriction applies to are the protected SCADA-Zones and Firewall-Zones.}
\end{itemize}

We have outlined the design principles for constructing a single firewall-path in a network.
In actuality, these principles and methods apply equally when constructing device-paths in other policy contexts.

We define single firewall-path concatenation based on the above design principles

\begin{defn}[Single firewall-path concatenation]
Take $a \in F^* \  \text{s.t.} \ a=t_{d_1d_2}t_{d_2d_3}t_{d_3d_4}...t_{d_nd_{n+1}} \ \text{where} $
$\ t_{d_id_j} \in F$. Also take $b \in F^* \ \text{s.t.} \ b=s_{g_1g_2}s_{g_2g_3}s_{g_3g_4}...s_{g_mg_{m+1}}$
$\ \text{where} \ s_{g_ig_j} \in F$. Then firewall-path concatenation from $F^* \times F^* \rightarrow F^*$ is \\\\
%\vspace{-3mm}
$ab= \begin{cases}
  t_{d_1d_2}...t^n_{d_nd_{n+1}}s_{g_1g_2}...s^m_{g_mg_{m+1}} \ \text{if} \ d_{n+1} = g_1 \\
  \ \ \text{and} \ g_i \neq d_j; \ \forall i,j, \ i >1 \\
  \ \ \text{and} \ h(t_{d_id_j}) \neq h(s_{g_kg_l}); \ \forall i,j,k,l \\  
  \phi, \ \text{otherwise}.
 \end{cases} $
 \label{v}
\end{defn}
%\vspace{-2mm}
\noindent and  $a \phi=\phi a= \phi ; \ \forall a \in F^*$

%TODO: include proof in thesis but simply state the fact here
\iffalse
\begin{lem}
Firewall-path concatenation above is a binary operation that generates loop-free paths.
\end{lem}

\begin{proof} TODO
\end{proof}
\fi
\smallskip
Concatenation in Definition 3 is a binary operation that constructs only elementary firewall-paths.

Consider two directed-firewalls $X,Y$ with policies $p_X$ and $p_Y$ that accepts packet sets $R$ and $T$.
The resultant policy of the concatenated firewall-path $XY$ has an action similar to that of sequential firewalls and can be denoted as 
$(p_X \otimes p_Y)(s) = p_{R \cap T}(s)$ where $s$ is a packet sequence.
The resultant policy action also depends on the policy context,. For instance, with traffic measurement policies, 
the outcome is similar to that of serial arbiters- \ie $p_X \otimes p_Y = p_{R \cup T}$.

We define a set of directed-firewall paths as a union of elements in $F^*$. 
Again, consider our directed-firewalls $X,Y$ from before.
If these described two distinct paths, then
the resultant policy of the path union $X \cup Y$ is that of parallel firewalls, \ie
$(p_X \oplus p_Y)(s) = p_{R \cup T}(s)$ where $s$ is a packet sequence. This result is also context dependent,
so, for traffic measurement policies, the outcome is similar to that of parallel arbiters, \ie
 $p_X \oplus p_Y = p_{R \cap T}$.

We also extend concatenation in Definition 2 to $S=\{\text{Power-set of } F^*\}$
\vspace{-1mm}
\begin{defn}[Multiple firewall-path concatenation]
Take $a,b \in S \  \text{s.t.} \ a=\{a_0,a_1...,a_x\}, b=\{b_0,b_1,...,b_y\} \ \text{where} \ a_i, b_j \in F^*$.
Then firewall-path concatenation from $S \times S \rightarrow S$ is given by

\smallskip
\indent \indent \indent \indent $ab= \{a_ib_j\}; \ \forall ij$  
 \label{v}
\end{defn}

%\vspace{-5mm} 
\noindent Then, Definition 3 allows all possible sets of firewall paths
to be constructed from the union of elements in $S$ (\ie $\forall a,b \in S, \ a \cup b \in S$).
Then $(S,\cup,\cdot,\hat{0},\hat{1})$ is an idempotent semiring with

\smallskip
$\hat{0}=\phi; \ \text{empty set}$; and

$\hat{1}=\{\epsilon\}; \ \text{empty-string set}$ where
$\epsilon$ is the identity element of the concatenation operation.

%TODO: include somewhere??
\iffalse
\smallskip
where $\epsilon$ is the identity element of the concatenation operation ({\ie empty string}) such that

$|\epsilon|=0$ and $\epsilon . s = s . \epsilon = s; \ \forall s \in F$.
\fi
\smallskip
\noindent It is important to note here that the properties of the operators $\cup$ and $\cdot$ actually dictate rules for firewall-path construction. 
So, when valid firewall-paths are built, they must be composed in a way that preserves these semantics. 
For instance, $\cup$ is commutative while $\cdot$ is not. So, the order of the directed-firewalls matter, when constructing a single firewall-path, but, are irrelevant
when constructing multiple paths.

Similarly, we can construct single and multiple device-paths for other policy contexts and
obtain the semiring result for $(S,\cup,\cdot,\hat{0},\hat{1})$ per security policies.

%Mapping policies to the network firewalls is now a matter of 
%finding a mapping from the directed-conduits in the Zone-Conduit graph to $S$, \ie
%we need to find a mapping $g : DC \rightarrow S$.
\vspace{-2mm}
\subsection{Mapping Policy to Arbiters}
\vspace{-2mm}
In the previous section we described how the semiring $(S,\cup,\cdot,\hat{0},\hat{1})$ constructs sets of device-paths between policy-graph endpoints.
The sequential (\ie $\otimes$) and parallel (\ie $\oplus$) policy-composition operators in \autoref{sec:abstractions} can now be used to construct the policies of these paths.
For instance,  assume we have to implement a high-level policy $p_{ij}$ on arbiters $q_{kl}$ that lie in the paths from $i$ to $j$.
All applicable device-paths from $i$ to $j$ can be constructed as per \autoref{sec:encoding} and given by
$S_{ij}=\{q_{a_1a_2}q_{a_2a_3}...q_{a_{n-1}a_n}, ....., q_{b_1b_2}q_{b_2b_3}...q_{b_{m-1}a_m}\}$.
Then, the high-level policy $p'_{ij}$ derived from the individual arbiter policies $p'_{kl}$ is
%\vspace{-2mm}
\begin{eqnarray}
  \label{eq:s2}
  p'_{ij}&=&(p'_{a_1a_2}\otimes p'_{a_2a_3}...\otimes p'_{a_{n-1}a_n}) \nonumber\\
  &&\oplus \  (....................................) \nonumber \\
  &&\oplus \ (p'_{b_1b_2} \otimes p'_{b_2b_3}...\otimes p'_{b_{m-1}b_m}).
\end{eqnarray}
\indent Mapping the intended high-level policy $p_{ij}$ to the arbiters is now a matter of finding $p'_{ij}$ for all arbiters such that
$p'_{ij}=p_{ij}$. But deriving such a mapping is non trivial because the meaning of $\oplus$ and $\otimes$ depends on the policy context.
For instance, with security policies $\oplus$ means {\em union} and $\otimes$ means {\em intersection}. So, a simple solution that supports {\em defence in depth} would be to implement the access-control policy $p_{ij}$ on every sequential firewall across all paths.\\
\indent For another instance, $\oplus$ means {\em summation} and $\otimes$ means {\em minimum} in QoS policies. So, a required bandwidth guarantee $p_{ij}$ can be split across multiple paths with sequential arbiters in each path guaranteeing only a portion of the total bandwidth.\\
\indent Similarly, with traffic measurement policies, $\oplus$ means {\em intersection} and $\otimes$ means {\em union}. So, each path must implement policy $p_{ij}$.
This can be achieved in multiple ways: (i) we could implement $p_{ij}$ on every sequential arbiter of a path for redundancy; or (ii) efficiently have only one arbiter per path implementing the policy; or
(iii) find an intermediate solution by partitioning $p_{ij}$ between sequential arbiters in a path.\\
\indent Irrespective of the policy context, the underlying requirement when mapping policy to network devices is to adhere to the semantics of \autoref{eq:s2}.
% how can we find this?
% for security policies - plus: union, times-intersection: ie for defece in depth, we consider all paths, and we implement policy on every sequentially composed arbiter
% so for security policies we implement p'_{a_ua_v}=p'_{b_xa_y}= p'_{ij} \forall u,v,x,y
% but for other policy contexts this will be different
% for example QoS: plus:sum  times- min- ie the required bw guarantee can be split across the multiple paths and each path must provide a min bw guarantee of the split amount. For instance, in current context....
% traffic measurement- plus: intersection  times: union - ie so each path must implement HL policy, for redundancy we could implement policy on every arbiter in a path or for efficiency have only one arbiter implement it
%or have an intermediate sol by partitioning the HL policy between the arbiters along one path. For instance, in current context....
\vspace{-2mm}
\subsection{Computation of All Firewall-paths}
\label{sec:calc}
\vspace{-3mm}
We have managed to reduce the policy-to-device mapping problem to the semantics of \autoref{eq:s2} in the previous section.
We now describe how an algorithm can be developed to compute the device-paths of \autoref{eq:s2} efficiently.
Again, we demonstrate the idea using security policies and the Zone-Conduit model.
%We now describe how the operators defined in the previous section and the results that followed can be used 
%to precisely compute all valid device-paths between {\em every pair of endpoints} in the policy-graph.

We can represent the firewall-paths of the primary-conduits using a {\em generalised Adjacency matrix $A$}. 
Here, $A(i,j)$ is the firewall-path of primary conduit $C_{ij} \in DC$. For our example in Figure \autoref{fig:vcf51}, $A=$
\smallskip

\begin{equation}
\begin{matrix}
  \begin{bmatrix}
  \overmat{$Z_1$}{\{\epsilon\}} & \overmat{$Z_2$}{\{A_{12},B_{12}\}} & \overmat{$Z_3$}{\phi} & \overmat{$Z_4$}{\{E_{14}\}} \\
  \{A_{21},B_{21}\} & \{\epsilon\} & \{C_{23},D_{23}\} & \phi \\
  \phi & \{C_{32},D_{32}\} & \{\epsilon\} & \{F_{34},G_{34}\} \\
  \{E_{41}\} & \phi & \{F_{43},G_{43}\} & \{\epsilon\} \\  
  \end{bmatrix}
\end{matrix}
\end{equation}

 Given such a matrix $A$, the solution to the problem of finding the set of all {\em valid}
 firewall-paths between zones is a matrix $A^*$ such that
 \begin{eqnarray}
  \label{eq:s3}
  A^*(i,j)&=&\{ \text{valid primary- and secondary-conduit} \nonumber \\
 &&\text{firewall-paths from zone i to j}\}
\end{eqnarray}

%TODO: talk about how our algorithm differs from the meta routing ones
We developed the following right iteration algorithm\footnote{See appendix for proof.} to compute $A^*$, 
inspired by algorithms in meta-routing \cite{griffin2013}.
In doing so, we allow the node property: {\em traffic transitivity}, to be explicitly specified via a {\em zone-transitivity} matrix $T$.
\begin{eqnarray}
  \label{eq:s4}
 A^{<0>}&=&I \nonumber \\ 
 A^{<k+1>}&=&({A^{<k>} T} \ \cup \ I) A
\end{eqnarray}

The {\em zone-transitivity} matrix $T$ is defined as
\begin{equation}
  \label{eq:p}
  T(i,j)= 
  \begin{cases}
  \{\epsilon\} \ \text{if} \  i=j \ \text{and} \ \text{zone\_transitivity}(i)=1\\
  \phi, \ \text{otherwise}.
  \end{cases}
\end{equation} 

and $I$ is the multiplicative-identity matrix

\begin{equation}
  \label{eq:h}
  I(i,j)= 
  \begin{cases}
  \hat{1} \ \text{if} \  i=j \\
  \hat{0}, \ \text{otherwise}.
  \end{cases}
\end{equation} 

\smallskip
%TODO: include proof of this in thesis!
For bounded semirings we only iterate $n-1$ times to converge to $A^*$, where $n$ is the number of nodes in the Zone-Conduit model, \ie

\smallskip
\indent \indent  $A^*=A^{<n-1>}$

\smallskip
We have defined $T$, $A^*$ and the right-iteration algorithm for a security-policy context, but these can equally be defined for other policy contexts.
%Generically, $T$ would be the {endpoint-transitivity} matrix defined similar to \autoref{eq:p}, $A^*$ would hold the set of all valid device-paths between endpoints,
%and calculated via \autoref{eq:a1}.

If we apply our algorithm in \autoref{eq:s4} to the example in Figure \autoref{fig:vcf51}, $n=4$, so, $A^*=A^{<3>}$ and let's {\em assume for simplicity that all zones are transitive}. Then

\begin{equation}
\begin{matrix}
  T=
  \begin{bmatrix}
  \{\epsilon\} & \phi & \phi & \phi \\
  \phi & \{\epsilon\} & \phi & \phi \\
  \phi & \phi & \{\epsilon\} & \phi \\
  \phi & \phi & \phi & \{\epsilon\} \\
 \end{bmatrix}
\end{matrix}
\end{equation}

and we see that $I=T$ in this instance.
%\smallskip
\begin{eqnarray}
  \label{eq:s5}
 A^{<1>}&=&({A^{<0>} T} \ \cup \ I) A=({I T} \ \cup \ I) A \nonumber \\ 
 &=&(I \ \cup \ I)A=A \nonumber \\
 A^{<2>}&=&({AT} \ \cup \ I)A \nonumber
\end{eqnarray}

\iffalse
\begin{equation}
\begin{matrix}
  \begin{bmatrix}
  \{\epsilon\} & \{A_{12},B_{12}\} & \alpha & \{E_{14}\} \\
  \{A_{21},B_{21}\} & \{\epsilon\} & \{C_{23},D_{23}\} & \beta \\
  \gamma & \{C_{32},D_{32}\} & \{\epsilon\} & \{F_{34},G_{34}\} \\
  \{E_{41}\} & \delta & \{F_{43},G_{43}\} & \{\epsilon\} \\
 \end{bmatrix}
\end{matrix}
\end{equation}

where for instance

\smallskip
\noindent $\beta=\{A_{21}E_{14},B_{21}E_{14},C_{23}F_{34},C_{23}G_{34},D_{23}F_{34},D_{23}G_{34}\}$.
\fi
%\noindent $\alpha=\{A_{12}C_{23},A_{12}D_{23},B_{12}C_{23},B_{12}D_{23},E_{14}F_{43},E_{14}G_{43}\}$.
%\indent \indent  $\gamma=\{C_{32}A_{21},C_{32}B_{21},D_{32}A_{21},D_{32}B_{21},F_{34}E_{41},G_{34}E_{41}\}$
%\indent \indent  $\delta=\{E_{41}A_{12},E_{41}B_{12},F_{43}C_{32},F_{43}D_{32},G_{43}C_{32},G_{43}D_{32}\}$

\smallskip
So, $A^*=A^{<3>}=({A^{<2>} T} \ \cup \ I) A=$

\begin{equation}
\begin{matrix}
  \begin{bmatrix}
  \{\epsilon\} & \eta & \kappa & \theta \\
  \mu & \{\epsilon\} & \nu & \beta \\
  \gamma & \lambda & \{\epsilon\} & \rho \\
  \xi & \delta & \zeta & \{\epsilon\} \\
 \end{bmatrix}
\end{matrix}
\end{equation}
where for instance
\begin{eqnarray}
  \label{eq:e}
 \kappa&=&\{A_{12}C_{23},A_{12}D_{23},B_{12}C_{23},B_{12}D_{23},E_{14}F_{43} \nonumber \\ 
 &&E_{14}G_{43}\} 
\end{eqnarray}

All valid firewall-paths from zone 1 to 3 are in $\kappa$.

%\smallskip
%\noindent $\kappa=\{A_{12}C_{23},A_{12}D_{23},B_{12}C_{23},B_{12}D_{23},E_{14}F_{43},E_{14}G_{43}\}$

%\indent \indent $\eta=\{A_{12},B_{12}, E_{14}F_{43}C_{32}, E_{14}F_{43}D_{32}, E_{14}G_{43}C_{32},$
%\indent \indent \indent \indent \indent $\ E_{14}G_{43}D_{32}\}$

%\indent \indent $\theta=\{E_{14},A_{12}C_{23}F_{34},A_{12}C_{23}G_{34},B_{12}C_{23}F_{34},B_{12}C_{23}G_{34},$
%\indent \indent \indent \indent $A_{12}D_{23}F_{34},A_{12}D_{23}G_{34},B_{12}D_{23}F_{34},B_{12}D_{23}G_{34}\}$

%\indent \indent $\mu=\{A_{21},B_{21},C_{23}F_{34}E_{41},C_{23}G_{34}E_{41},D_{23}F_{34}E_{41},$
%\indent \indent \indent \indent \indent $\ D_{23}G_{34}E_{41}\}$

%\indent \indent $\nu=\{C_{23},D_{23},A_{21}E_{14}F_{43},A_{21}E_{14}G_{43},B_{21}E_{14}F_{43},$
%\indent \indent \indent \indent \indent $\ B_{21}E_{14}G_{43}\}$

%\indent \indent $\lambda=\{C_{32},D_{32},F_{34}E_{41}A_{12},F_{34}E_{41}B_{12},G_{34}E_{41}A_{12},$
%\indent \indent \indent \indent \indent $\ G_{34}E_{41}B_{12}\}$

%\indent \indent $\rho=\{F_{34},G_{34},C_{32}A_{21}E_{14},C_{32}B_{21}E_{14},D_{32}A_{21}E_{14},$
%\indent \indent \indent \indent \indent $\ D_{32}B_{21}E_{14}\}$

%\indent \indent $\xi=\{E_{41},F_{43}C_{32}A_{21},F_{43},C_{32}B_{21},F_{43},D_{32}A_{21},F_{43},D_{32}B_{21},$

%\indent \indent \indent \indent $G_{43}C_{32}A_{21},G_{43}C_{32}B_{21},G_{43}D_{32}A_{21},G_{43}D_{32}B_{21}\}$

%\indent \indent $\zeta=\{F_{43},G_{43},E_{41}A_{12}C_{23},E_{41}A_{12}D_{23},E_{41}B_{12}C_{23},$
%\indent \indent \indent \indent \indent $\ E_{41}B_{12}D_{23}\}$

% not required for this paper (include in the reasoning language paper)
\iffalse
\smallskip
Also, let $S^*=\text{Kleene Star of } S$

\indent \indent \indent \indent $=\{\{\epsilon\}, \{A_{12}\}, \{B_{12}\}, \{A_{21}\},...,\{A_{12},B_{12}\}, \{A_{12}C_{23}\}$

\indent \indent \indent \indent \indent $\{A_{12}B_{12},A_{12}C_{12}\},..\}$

\indent \indent \indent $1 \oplus (SS^*)=\{\epsilon\} \oplus \{\{\epsilon\}, \{A_{12}\}, \{B_{12}\}, \{A_{21}\},...$

\indent \indent \indent \indent \indent \indent   $,\{A_{12},B_{12}\}, \{A_{12}C_{23}\},\{A_{12}B_{12},A_{12}C_{12}\},...\}$

\indent \indent \indent \indent \indent \indent \indent \indent $ =S^*$

Similarly \indent \indent \indent $1 \oplus (S^*S)=S^*$

So, $(S,\oplus,.,*,0,1)$ is a Kleene Algebra.
\fi

\smallskip
Let's now {\em assume that zone \verb|4| is non-transitive}, then $zone\_transitivity(4)=0$, and by \autoref{eq:p}, 

\begin{equation}
\begin{matrix}
  T=
  \begin{bmatrix}
  \{\epsilon\} & \phi & \phi & \phi \\
  \phi & \{\epsilon\} & \phi & \phi \\
  \phi & \phi & \{\epsilon\} & \phi \\
  \phi & \phi & \phi & \phi \\
 \end{bmatrix}
\end{matrix}
\end{equation}

We re-calculate $A^*=$

\begin{equation}
\begin{matrix}
  \begin{bmatrix}
  \{\epsilon\} & \{A_{12},B_{12}\} & \eta & \theta \\
  \{A_{21},B_{21}\} & \{\epsilon\} & \{C_{23},D_{23}\} & \mu \\
  \gamma & \{C_{32},D_{32}\} & \{\epsilon\} & \rho \\
  \xi & \delta & \zeta & \{\epsilon\} \\
 \end{bmatrix}
\end{matrix}
\end{equation}

where for instance
\begin{eqnarray}
  \label{eq:s6}
 \eta=\{A_{12}C_{23},A_{12}D_{23},B_{12}C_{23},B_{12}D_{23}\}
\end{eqnarray}

%\smallskip
%\indent \indent $\eta=\{A_{12}C_{23},A_{12}D_{23},B_{12}C_{23},B_{12}D_{23}\}$.

\smallskip
The updated firewall-paths from 1 to 3 are in $\eta$. In comparison to \autoref{eq:e},
we see that the paths via zone 4 (\ie $E_{14}F_{43},E_{14}G_{43}$) have now been removed as the zone is no longer transitive.
$A^*$ can similarly be calculated for other policy contexts to determine all valid device-paths between endpoint pairs.

\smallskip
\noindent We will next describe our implementation of the algorithm in \autoref{eq:s4}. 
The implementation allows us to use these algebras to map policy to real network devices.
\vspace{-5mm}

==> Firewall path algebra - tech report/background.tex <==
\section{\uppercase{Background and Related work}}
\label{sec:background}
\vspace{-5mm}
% most networks are build using a bottom-up configuration approach
\smallskip
\begin{myquote}{Bertrand Russel}
``The advantages of implicit definition over construction are roughly those of theft
over honest toil.''
\end{myquote}

The quote is salient because network installations are commonly built from {\em bottom-up}, 
\ie a network-device is purchased, and configurations written. The policy is the result of the configuration, which is the
consequence of a purchasing decision. So, the policy is implicitly defined as a result of many small decisions
that interact in complex ways. Instead, best-practice guides \cite{byres2005,isa2007} suggest designing the policy first, and only then
determining how to implement it. 

% what should be used instead is a top-down configuration approach with high-level policies
Solutions that employ such a {\em top-down} network configuration approach have been proposed in both 
\ac{SDN} \cite{soule2014,anderson2014,prakash2015} and traditional networks \cite{bartal1999,cisco2014b}. 
They allow creation and maintenance of a {\em single high-level network-wide policy}
(\ie source of truth), so network administrators can easily determine, for instance,
who gets in and who doesn't. These high-level policies should be decoupled from
network and device-vendor intricacies, so they capture the {\em policy intent} and not the {\em policy implementation}.

Capturing intent has several benefits: it allows policy to be distinguished from network to assist with change management;
it enables accurate comparison of organisational policies to industry best-practices to evaluate compliance; and
it allows policy semantics to be expressed without network intricacies like IP addresses.
But, most research towards high-level policy languages \cite{bartal1999,cisco2014b,soule2014}, still requires hostnames and/or IP addresses to be
explicitly input to the policy specification, to implement policy on a network instance.

% policies need to have formal semantics
If the high-level policy definition is built on {\em formal mathematical constructions}, then
there are no implicit properties and it provides a truly sound foundation for everything that follows. 
The formalism would allow construction of complex and flexible policies and support reasoning about the policies.
For instance, we could precisely compare a defined policy with industry best-practices in \cite{isa2007,byres2005} for compliance and reduce 
network vulnerability to cyber attacks \cite{ranathunga2015P}. 

% and formal mapping framework
It is equally important to map policy to devices using a formal approach.
For instance, we can be confident of the blanket of protection
provided for our network {\em if and only if} we could prove that an intended security policy is implemented by the correct set of network firewalls.
Existing top-down configuration languages \cite{bartal1999,prakash2015,cisco2014b} allow creation of network-wide high-level policies, but
lack means to allocate policy to network devices in provably correct way.

In our related work \cite{ranathunga2015V}, we have developed a high-level security policy specification 
that is network and device-vendor independent
to perform {\em top-down} configuration of network firewalls.
The language semantics allow these high-level policies to be
easily understood by humans. 
In this paper, we investigate the underlying requirements for
mapping high-level policy to network devices.
\vspace{-6mm}

==> Firewall path algebra - tech report/conclusion.tex <==
\section{\uppercase{Conclusions}}
\label{sec:conclusion}
\vspace{-2mm}
There are various obstacles that hinder the precise mapping of policies to network devices.
Most prominent is the lack of decoupling between policy and network which makes
policy sensitive to network-intricacies and vendor changes.
To compound the problem, policies can also have complex
semantics including node and link properties.

Our research addresses these challenges and proposes
a mathematical foundation for mapping policies to network-devices.
We use it to deploy real-world security policies to network firewalls
provably correctly, so, that administrators can be confident of the protection provided by their policies for their networks.
\vspace{-7mm}



==> Firewall path algebra - tech report/implementation.tex <==
\section{\uppercase{Implementation}}
\label{sec:imp}
\vspace{-2mm}
Our policy mapping system is depicted in \autoref{fig:map}, and we outline it's details below.
The system is currently implemented in Python, and allows mapping of high-level policies written in our
own policy specification language, to network devices. We will make the system open source in the near future.

%\smallskip
\noindent \textbf{\em High-level security policy:} The topology-independent policy input file created using our high-level policy specification language.

%\smallskip
\noindent \textbf{\em Network topology:} The input network topology described in the XML-based graph file format {\em GraphML} \cite{GraphML}.
The file holds information of all devices in the network and their interconnections. The crucial aspects are the details of the
topology near the policy arbiters (\eg firewalls).

%\smallskip
\noindent \textbf{\em Map policy to network:} Compiles high-level policy to an Intermediate-Level (IL), generates the policy graph (\eg Zone-Conduit model) of the input network and computes $A^*$ as per \autoref{sec:calc} to map high-level policy to the devices (\eg firewalls) in the network.

%\smallskip
\noindent \textbf{\em Policy-to-device map:} The primary output depicting policy breakdown by device, interface and direction.

%\smallskip
\noindent \textbf{\em Verification output:} Secondary output specifically suited for verification (\eg policy errors).
\begin{figure}[t!]
%\center
\captionsetup{aboveskip=8pt}
\centerline{\includegraphics[scale=0.35]{policy_mapper.pdf}}
\caption{Policy to network-device mapping process.}
\label{fig:map}
\end{figure}

\smallskip
\noindent Our system implements a high-level policy on a network by coupling the policy to the topology instance. 
Details of the coupling steps are discussed in detail in our previous work in \cite{ranathunga2015V}.
We outline here, the steps taken to map policy to the network devices. Again, we illustrate our implementation 
using security policies and the Zone-Conduit model, but the system can likewise be used in other policy contexts.
\vspace{-2mm}
\subsection{Zone-transitivity Matrix and Adjacency Matrix Construction}
%\subsection{Zone-Conduit Model Construction}
%\label{sec:zone-cond-gen}
\vspace{-2mm}
Our system first builds the \textit{Zone-Firewall model}, containing the disjoint zones and their 
firewall interconnections using the input network topology. 
Additional Firewall-Zones, Abstract-Zones and Carrier-Zones \cite{ranathunga2015} are added to the model as required. 
The primary conduits are then defined to create the Zone-Conduit model. 
%\vspace{-2mm}
%\vspace{-2mm}

Next, the zone-transitivity capabilities are collated by compiling the high-level policy to IL policy.
Then the $n \times n$ zone-transitivity matrix ($T$) is constructed ($n$ is the number of zones in the network). 

Implicit mappings between the primary conduits and their firewall compositions are automatically created when generating the Zone-Conduit model. 
These mappings are leveraged to construct the adjacency matrix $A$ described in \autoref{sec:calc}.
\vspace{-2mm}
\subsection {$A^*$ Calculation}
\vspace{-2mm}
We compute $A^*$ using the right iteration algorithm in \autoref{eq:s4}.
Our implementation is given below (Algorithm 1). 
We consider a centralised implementation (given typically low $n$), but, it can also be 
distributed across multiple nodes performing parallel computations.

\begin{table*}[t]
\caption{SCADA case study summary adapted from \cite{ranathunga2015} ($*$ includes backup firewalls, $\#$ ACL rule allocation error).} % title of Table
\centering % used for centering table
\begin{tabular}{c l c c c c c c c c c c} % centered columns (4 columns)
\hline\hline %inserts double horizontal lines
SUC & \multicolumn{1}{p{1cm}}{\centering Config. \\ date} & \multicolumn{1}{p{0.6cm}}{\centering Fire-walls$^*$} &  \multicolumn{1}{p{0.65cm}}{\centering Zones}  & \multicolumn{1}{p{1cm}}{\centering Conduits} &  \multicolumn{1}{p{0.8cm}}{\centering Max. \\ hosts} &
\multicolumn{1}{p{0.55cm}}{\centering ACLs} & \multicolumn{1}{p{1.25cm}}{\centering Average rules \\ per ACL } & \multicolumn{1}{p{1.1cm}}{\centering Incorrect \\ firewall$^{\#}$ } & \multicolumn{1}{p{1.1cm}}{\centering Incorrect \\ interface$^{\#}$} & \multicolumn{1}{p{1.1cm}}{\centering Incorrect \\ direction$^{\#}$} & \multicolumn{1}{p{1.1cm}}{\centering Runtime \\ (seconds)}  \\ [0.5ex] % inserts table
%heading
\hline % inserts single horizontal line
1 & Sep 2011 & 3  & 7 &11 & 67580 & 8 & 237 & 15  & 13 & 19 & 40 \\ % inserting body of the table
2 & Aug 2011 & 6 & 21 & 81 & 2794 & 12 & 16 & 3 & 2 & 5 & 70\\
3 & Oct 2011 &  4 & 10 & 17 & 886 & 8 &  6 & 2 & 1 & 4 & 43\\ 
4 & Mar 2011 &  3 & 9 & 16 & 2038 & 3 & 80 & 5 & 12 & 13 & 61\\
5 & Apr 2015 &  3 & 12 & 19 & 2664 & 12 & 677 & 15 & 8 & 26 & 47\\
6 & Apr 2015 &  3 & 13 & 21 & 3562 & 8 & 1034 & 21 & 15 & 19 & 63\\
7 & Jul 2015 &  6  & 15 & 22 & 3810 &  17 & 724 &  9 & 5 & 17 & 49\\
\hline %inserts single line
\end{tabular}
\label{table:suc-summary} % is used to refer this table in the text
\end{table*}

\begin{algorithm}[t]
\caption{Right-iteration algorithm to compute $A^*$.
The additive and multiplicative operators of Semiring $S$ are $\cup, \cdot$ (\autoref{sec:encoding}).
The additive and multiplicative identities of $S$ are $\hat{0}, \hat{1}$. 
The multiplicative-identity matrix and the zone-transitivity matrix are $I$ and $T$.
The set of zones in the network is $Z$.}
\label{alg:right_iter}
\begin{algorithmic}[1]
\Procedure{RightIteration}{$(\cup, \cdot, \hat{0}, \hat{1},A)$}
\State $R_0 \gets \text{I}$
\State $k \gets \text{1}$

\While{$k \leq |Z| -1$}
	\ForEach{$i \in Z$}
		\ForEach{$j \in Z$}
		      \If{i=j} 
		      	  \State $R_{k+1}(i,j) \gets I(i,j)$
		      \Else
		          \State $R_{k+1}(i,j) \gets \hat{0}$
		          \ForEach{$q \in Z$}
		               \State $s \gets R_k(i,q) \cdot T(q,j)$
		               \State $R_{k+1}(i,j) \gets R_{k+1}(i,j) \cup s$		               
		               \State $R_{k+1}(i,j) \gets R_{k+1}(i,j) \cup I(i,q)$
		               \State $R_{k+1}(i,j) \gets R_{k+1}(i,j) \cdot A(q,j)$
		          \EndFor
		      \EndIf
		\EndFor
	\EndFor
	\State $k \gets \text{k+1}$
 \EndWhile
\EndProcedure
\end{algorithmic}
\end{algorithm}
%\vspace{-1mm}
Lines 2,3,10 initialise $R_0$, $k$ and $R_{k+1}(i,j)$ while lines 5,6,11 range over the set of zones $Z$ in the network.
At each step $k$, we store the result $A_{k+1}$ in $R_{k+1}$.

% talk about O(n4) time complexity - n < 100 in a typical SCADA network so this is manageable, network-grouping can keep N small as opposed to
% specifying policy per host
We can see that the above algorithm has time complexity $O(n^4)$. This value suggests that the algorithm performance decreases exponentially as the number of zones in the network ($n$) increases.
So, specifying policy per individual host (\ie zone size=1 so, large $n$) in {\em top-down} configuration makes policy mapping {\em extremely inefficient}. 
It proves more efficient to create network groups (\eg by subnet) and specify policy between them, so, a reasonably low value can be maintained for $n$.
For instance, we will see in \autoref{sec:example} that in a SCADA network typically $n< 25$. 
Our mapping algorithm runs on average in 53 seconds 
on a standard desktop computer for each of these networks.
%So, the average time taken by our policy mapping algorithm to run
%on a standard desktop computer is 53 seconds for these networks.
%(\eg Intel Core CPU 2.7-GHz computer with 8GB of RAM running Mac OS X), 

%TODO: this is also important (do we extend our algebra to support these policy allocation strategies?)
%understanding the device-paths that need to implement policy is one thing (whether all paths or subset of all paths)
%determining a suitable policy allocation strategy for the devices in the individual paths is another thing
%  . do we allocate policy uniform to each device in a path? (eg with security policies this yields defence in depth) or only to edge devices? (more efficient but single point f faiure) or several (not all) devices in a path (semi defence in depth)?
% all paths vs pruned paths
In calculating $A^*$, we considered all valid paths between two zones (hence time complexity of $O(n^4)$). The decision allows us to permit or block traffic along all possible communication paths between two zones, providing redundancy and {\em defence-in-depth} in the network. 
We also map policy uniformly to every firewall along a single-path, further boosting defence-in-depth.
These decisions collectively create a more robust defence against cyber attacks. 

However, in other policy contexts, it may be useful to select a {\em subset} of all valid paths or even just a single path (\eg shortest path) instead.
Doing so, could improve the time complexity of \autoref{eq:s4} (\eg selecting shortest paths would yield $O(n^3)$).
This path pruning can be done, for instance, by incorporating a sparse matrix in \autoref{eq:s4}.
It may also be efficient to apply policy only on edge arbiters of a path, in some contexts (\eg when enabling traffic measurements).
\vspace{-7mm}

==> Firewall path algebra - tech report/introduction.tex <==
\section{\uppercase{Introduction}}
\label{sec:introduction}
\vspace{-2mm}
% Top-down network configuration is essential. It requires the ability to specify HL network-wide policies.
Managing modern-day networks is complex, tedious and error-prone. These networks are comprised of  a wide variety of devices, from switches and routers to middle-boxes  like firewalls, intrusion detection systems and load balancers. Configuring these heterogeneous devices with their potentially complex policies manually, box-by-box is impractical.

A better approach is a {\em top-down configuration} where device configurations are derived from a high-level user specification. 
Such specifications raise the level of abstraction of network policies above device and vendor-oriented APIs (\eg Cisco CLI, OpenFlow). 
Doing so, provides {\em a single source of truth}, so, security administrators for instance, can easily determine who gets in and who doesn't \cite{howe1996}. 

In recent years, several research groups have proposed high-level policy specification languages for both \ac{SDN} \cite{soule2014,reich2013,foster2010,prakash2015} 
and traditional networks \cite{bartal1999,guttman2005}.
A common requirement in these languages is the ability to map the abstract policies to the underlying physical network. Doing so accurately, is essential to:
%\vspace{-1mm}
\begin{itemize}
\item enforce policy correctly;
\vspace{-1mm}
\item track policy changes per network device, so, redundant policy updates can be avoided; 
\end{itemize}
\smallskip
But, mapping policies to the physical network devices has challenges:

\begin{itemize}
 
\item policy needs to be {\em decoupled} from the network (\ie free of vendor and network-centric minutiae). A policy shouldn't need to change when
the device vendor changes, or every time IP address changes occur;
\vspace{-1mm}
\item the mapping must be {\em formally verifiable}. Precise and unambiguous mathematical semantics would eliminate wishful thinking pitfalls in deploying policies to networks. These semantics give, for instance, security administrators assurance that their intended policies are enforced by the correct
firewalls, rendering the expected security outcome.
%For instance, with security policies, administrators need assurance that the policies are enforced by the correct devices and they provide the expected security outcome;
\vspace{-1mm}
\item policies can have complex semantics including node and link properties; and
\vspace{-1mm}
\item the mapping should be as efficient as possible.
%\item translating high-level policy to network-level and then mapping to the network devices is inefficient;
%\item policy best-practices such as 'prohibit traffic transiting through a protected \ac{SCADA} network' \cite{byres2005} need to be adhered to, when implementing policy on devices.
%\item  certain network segments can impose additional constraints that need to be accounted for when implementing policy on the network (\eg a protected SCADA network restricts traffic that can transit it \cite{byres2005});
%\item deriving a uniform mapping model for both SDN and traditional networks is non trivial (mapping policy to a set of switches is sufficient in SDN whereas traditional networks may need mapping to a device-interface level);
\end{itemize}

% our solution - we enable HL filtering policies (main focus) without network intricacies based on z-c abstraction, we map HL policy directly to network devices using the z-c model	
The solution we propose provides a generic framework to map policies to network devices algebraically. 
We illustrate it's use by considering security policies, 
because incorrect deployment of these policies in domains such as \ac{SCADA} networks can result in
catastrophic outcomes including the loss of human lives!
However, the principles involved, can easily be extended to policies involving traffic measurement, QoS, load balancing and so on. 

In developing our algebras, we have derived the properties and constraints of sequentially- and parallelly-composed policies for various policy contexts.
These policy-composition semantics must be preserved, when mapping policy to devices, to ensure correct deployment.
Using an algebraic framework also makes the policy-mapping process efficient.

We will describe the implementation of our proposed algebras and demonstrate their use in deploying security policies to real SCADA networks.
Particularly, we will show it's value in maintaining a clear, concise set of firewall configurations.
Moreover, our approach allows administrators to conduct ``what if'' analysis by changing policy and/or network topology 
and observe their effect on the network devices required to implement the changes.
\vspace{-6mm}
